COUCH: Towards Controllable Human-Chair Interactions

Humans interact with an object in many different ways by making contact at different locations, creating a highly complex motion space that can be difficult to learn, particularly when synthesizing such human interactions in a controllable manner. Existing works on synthesizing human scene interaction focus on the high-level control of action but do not consider the fine-grained control of motion. In this work, we study the problem of synthesizing scene interactions conditioned on different contact positions on the object. As a testbed to investigate this new problem, we focus on human-chair interaction as one of the most common actions which exhibit large variability in terms of contacts. We propose a novel synthesis framework COUCH that plans ahead the motion by predicting contact-aware control signals of the hands, which are then used to synthesize contact-conditioned interactions. Furthermore, we contribute a large human-chair interaction dataset with clean annotations, the COUCH Dataset. Our method shows significant quantitative and qualitative improvements over existing methods for human-object interactions. More importantly, our method enables control of the motion through user-specified or automatically predicted contacts.

==> COUCH - arxiv/Definitions.tex <==
%% Type definitions
% \usepackage{amsmath}
% \DeclareMathOperator*{\argmax}{arg\,max}

\newcommand{\model}[0]{COUCH}
\renewcommand{\vec}[1]{\boldsymbol{#1}}
\newcommand{\mat}[1]{\mathbf{#1}}
\newcommand{\set}[1]{\mathcal{#1}}
\newcommand{\vect}[1]{\mathbf{#1}}

%% SMPL definitions
\newcommand{\template}[0]{\mat{T}}
\newcommand{\blendweight}[0]{w}
\newcommand{\blendweights}[0]{\mat{W}}

% \newcommand{\pose}[0]{\vec{\theta}}
\newcommand{\shape}[0]{\vec{\beta}}
\newcommand{\trans}[0]{\vect{t}}
\newcommand{\joints}[0]{\mat{J}}
\newcommand{\offsets}[0]{\mathbf{D}}

\newcommand{\smpl}[0]{M}
\newcommand{\posefun}[0]{T}
\newcommand{\blendfun}[0]{W}
\newcommand{\offsetfun}[0]{B}
\newcommand{\jointfun}[0]{J}

\newcommand{\hist}[1]{{#1}^-_t}
\newcommand{\future}[1]{{#1}^+_t}

%% Commenting definitions
\newcommand{\BB}[1]{{\textcolor{purple}{[\textbf{BB:} #1]}}}
\newcommand{\GPM}[1]{{\textcolor{red}{[\textbf{GPM:} #1]}}}
\newcommand{\XZ}[1]{{\textcolor{blue}{[\textbf{XZ:} #1]}}}
\newcommand{\Seb}[1]{{\textcolor{magenta}{[\textbf{SS:} #1]}}}

%% Project specific definitions
%% Hand Control
\newcommand{\control}{\mat{C}} 
\newcommand{\contact}{\vec{c}}
\newcommand{\handtraj}{\mat{h}}
\newcommand{\handtrajinterp}{\mat{\tilde{h}}}
\newcommand{\localphase}{\mat{\phi}}
\newcommand{\globalphase}{\mat{\Phi}}

\newcommand{\handtrajpred}{{\dot{\mat{h}}}}
\newcommand{\localphasepred}{\dot{\mat{\phi}}}
\newcommand{\globalphasepred}{\dot{\mat{\Phi}}}

%% Motion Network
\newcommand{\poseposition}{\vec{j}^{p}_i}
\newcommand{\posevelocity}{\vec{j}^{v}_{i}}
\newcommand{\poserotation}{\vec{j}^{r}_{i}}
\newcommand{\poseacc}{\ddot{\vec{j}}_{i}}
\newcommand{\feettar}{\tilde{\vec{f}}_{i}}


\newcommand{\trajpos}{\vec{t}^{p}_{i}}
\newcommand{\trajdir}{\vec{t}^{d}_{i}}
\newcommand{\trajact}{\vec{t}^{a}_{i}}

\newcommand{\goalpos}{\vec{g}^{p}_{i}}
\newcommand{\goaldir}{\vec{g}^{d}_{i}}
\newcommand{\goalact}{\vec{g}^{a}_{i}}

\newcommand{\trajposgoal}{\tilde{\vec{t}}^{p}_{i}}
\newcommand{\trajdirgoal}{\tilde{\vec{t}}^{d}_{i}}

\newcommand{\pose}{\mat{J}}
\newcommand{\traj}{\mat{T}}
\newcommand{\goal}{\mat{G}}
\newcommand{\environment}{\mat{E}}
\newcommand{\scene}{\mat{I}}
\newcommand{\phase}{\phi}

% additional
\newcommand{\futureposeposition}{\vec{\tilde{j}}^{p}_{i+1}}
\newcommand{\goaltrajdir}{\vec{\tilde{t}}^{d}_{i+1}}
\newcommand{\goaltrajpos}{\vec{\tilde{t}}^{p}_{i+1}}

\newcommand{\goaltraj}{\mat{\tilde{T}}}
\newcommand{\binarycontact}{\vec{b}_{i+1}}


\newcommand{\x}{\mat{X}}
\newcommand{\y}{\mat{Y}}

\newcommand{\latent}{\vec{z}}

\newcommand{\expertweights}{\mat{\alpha}}


\newcommand{\myparagraph}[1]{\vspace{1pt}\noindent{\bf #1}}






